Comparing large language models for supervised analysis of students' lab notes

Recent advancements in large language models (LLMs) hold significant promise in improving physics education research that uses machine learning. In this study, we compare the application of various models to perform large-scale analysis of written text grounded in a physics education research classification problem: identifying skills in students' typed lab notes through sentence-level labeling. Specifically, we use training data to fine-tune two different LLMs, BERT and LLaMA, and compare the performance of these models to both a traditional bag of words approach and a few-shot LLM (without fine-tuning).} We evaluate the models based on their resource use, performance metrics, and research outcomes when identifying skills in lab notes. We find that higher-resource models often, but not necessarily, perform better than lower-resource models. We also find that all models estimate similar trends in research outcomes, although the absolute values of the estimated measurements are not always within uncertainties of each other. We use the results to discuss relevant considerations for education researchers seeking to select a model type to use as a classifier.

==> IssuesToConsider.tex <==
\section{Issues to consider}
\begin{itemize}
    \item How much resources do you have to devote to the project? - Computational, time, etc.    
    \item How much hyperparameter tuning do you have to do to make it work?  
    \item How much compute does a single train of the model take - do a chart with how much flops a single training run takes and how much the memory costs on gpu?
    \item How much labeled data do you need to get a decent model - do a graph of # of samples v.s. accuracy?
    \item What is the variance across different slices of data and random seeds for each method ?  
    \item What is the engineering (person time) cost?  
\end{itemize}

\subsection{Things I needed to change for the llama code to work }
\begin{itemize}
    \item  The original code was putting more on the GPU than necessary - which was overloading it when I moved up to a bigger model.   
    \item The original code uses a constant learning rate, whereas we get better results (and the consensus on Reddit lol) using a cosine scheduler.  
\end{itemize}

==> Metrics.tex <==
When human coders code data, they create a simple binary classification:  code or no code.
However, the machine learning models that we use here output a number between 0 and 1, corresponding to the model's estimation of the likelihood that the example belongs to the "code" class.  
This allows us to create an ordering of all the inputs from most to least likely to belong to the class (according to the model). 
To create a binary classification, the model employs a simple threshold:  Greater than .5 means it belongs to the "code" class. 
However, this ordering can be used before applying the threshold.  

We show in figure (?) that researchers can make different choices about their priorities for the model - Whether it matters more to catch all examples of the code (true positives a.k.a TP) or to prioritize accuracy, or some other metric.
We go into more detail about why one may choose each metric below.
Given the same ordering, we can maximize different performance metrics by changing the threshold.  
For our toy example, the threshold which maximizes each metric is shown in the figure.  
AUC, or area under the curve, is threshold-agnostic.  
For this case, the AUC corresponds to the probability that the model output will be higher for a randomly selected example of the code than for an example of "not code".  
This is 1 if the ordering is perfect, and .5 if the ordering is random.  





==> figures-data-code.tex <==

- make branch of current github that will be public
- make a clean jupyter notebook that produces the figures
     - at top of notebook, say that you can run bag of words here, and you can use this code to generate your own version of these log files, but that takes too long, use our log files
     - will contain 3-panel figure 1 (Accuracy, Balanced accuracy, and AUC)
     - will contain code that makes figure 2
     
- maybe add a separate jupyter notebook with same code that runs, toy example 
- before releasing code, add figure numbers
